Stationary Surfaces with Boundaries

This article investigates stationary surfaces with boundaries, which arise as the critical points of functionals dependent on curvature. Precisely, a generalized "bending energy" functional $\mathcal{W}$ is considered which involves a Lagrangian that is symmetric in the principal curvatures. The first variation of $\mathcal{W}$ is computed, and a stress tensor is extracted whose divergence quantifies deviation from $\mathcal{W}$-criticality. Boundary-value problems are then examined, and a characterization of free-boundary $\mathcal{W}$-surfaces with rotational symmetry is given for scaling-invariant $\mathcal{W}$-functionals. In case the functional is not scaling-invariant, certain boundary-to-interior consequences are discussed. Finally, some applications to the conformal Willmore energy and the p-Willmore energy of surfaces are presented.

==> 081-noscaleinvar_old.tex <==
% \section{\textbf{Functionals Without Scaling Invariance}}
\section{Functionals Without Scaling Invariance}

Many important functionals do not share the dilation-invariance seen in the Willmore energy.  It is easy to verify that even highly related measures such as the Helfrich-Canham energy (\ref{eq:helfrich}) do not remain static when a surface is rescaled.  Because of this, it is enlightening to also examine the properties of $\mathcal{W}$-functionals that are not scaling-invariant.  In particular, flux formula (\ref{eq:scaleflux}) can be used to show the following.

\begin{lemma}\label{lem:bndryctrl}
The equation
\begin{equation*}
    \int_\Sigma \left(2F - HF_H - 2KF_K\right)d\mu = 0,
\end{equation*}
holds for any $\mathcal{W}$-critical surface immersion $\*r(\Sigma)$ provided the following expressions hold on $\partial\Sigma$:
\begin{align}
    0 &= \tau_g F_H, \label{eq:bcond1} \\
    0 &= F - h(\con,\con)F_H -KF_K, \label{eq:bcond2} \\
    0 &= h(\nabla F_K,\con) - \nabla_\con F_H - H\nabla_\con F_K. \label{eq:bcond3}
\end{align}
% where $\kappa_n = h(\*T,\*T)$ and $\tau_g = h(\*T,\con)$ are the normal curvature and geodesic torsion of the boundary curve, respectively.
\end{lemma}

\begin{proof}
First, notice that $\nabla_\con \*r \perp \*n$, so that
\begin{equation*}
    \nabla_\con\langle \*r, \*n\rangle = \langle \*r, \nabla_\con \*n\rangle = -\left\langle \*r, \tau_g \*T + h(\con,\con)\con\right\rangle.
\end{equation*}
Also, writing $\nabla \langle \*r, \*n\rangle = \nabla_\*T \langle \*r, \*n\rangle \*T + \nabla_\con \langle \*r, \*n\rangle\con$, it follows that
\begin{equation*}
    h\left(\nabla\langle \*r, \*n\rangle, \con\right) = -\left\langle \*r, H\tau_g \*T + \left( \tau_g^2 + h(\con,\con)^2\right)\con \right\rangle.
\end{equation*}
With this, the right-hand side of equation  (\ref{eq:scaleflux}) becomes
\begin{align*}
&\int_{\partial \Sigma} \Big((F_H+HF_K)\nabla_\con \left\langle{\*r, \*n}\right\rangle - F_K h(\nabla \left\langle{\*r, \*n}\right\rangle, \con)\Big)\, ds\\
&+\int_{\partial \Sigma} \left\langle{\*r, \*n}\right\rangle\Big(h(\nabla F_K, \con)-\nabla_\con F_H-H\nabla_\con F_K\Big)\, ds + \int_{\partial \Sigma} F\left\langle{\*r, \con}\right\rangle \,ds \\
% &=\int_{\partial\Sigma} \left\langle \*r, -(F_H + H F_K)\left( \tau_g \*T + h(\con,\con)\con \right) + F_K H\tau_g \*T + F_K\left(\tau_g^2 + h(\con,\con)^2\right)\con \right\rangle\, ds \\
% &+ \int_{\partial\Sigma} \left\langle \*r, \left(h(\nabla F_K, \con)-\nabla_\con F_H-H\nabla_\con F_K\right)\*n \right\rangle\, ds + \int_{\partial\Sigma}\left\langle \*r, F\con\right\rangle\, ds \\
&= \int_{\partial\Sigma} \left\langle \*r, -\tau_g F_H \*T + \left(F - (F_H + H F_K)h(\con,\con) + \left(\tau_g^2 + h(\con,\con)^2\right)F_K\right)\con \right\rangle\, ds \\
&+ \int_{\partial\Sigma} \left\langle \*r, \left(h(\nabla F_K, \con)-\nabla_\con F_H-H\nabla_\con F_K\right)\*n \right\rangle \, ds.
\end{align*}
The inner product $\langle \*r,\*V\rangle$ inside the above integral expression vanishes for any immersion $\*r$ when each component of the vector field $\*V$ vanishes identically.  This combined with the fact that $H = h(\*T,\*T) + h(\con,\con)$ on $\partial\Sigma$ now yields the claimed boundary conditions.
\end{proof}

\begin{remark}
For immersions that meet a planar boundary tangentially, $\kappa_n = \tau_g = 0$ and the flux formula reduces to 
\[ \int_\Sigma \left(2F - HF_H - 2KF_K\right) d\mu = \int_{\partial\Sigma} (F-HF_H) \langle \*r,\con\rangle\, ds. \]  In the case where $F$ is the (scaling-invariant) Willmore functional, this implies the result of Dall'Acqua \cite{dall2012} that $h(\*X,\*Y) = 0$ for all vector fields $\*X,\*Y$ tangent to $\Sigma$ at the boundary.  More precisely, $\langle \*r, \con \rangle$ is of constant sign on $\partial\Sigma$, so it follows that $H \equiv 0$ there.  Since $\kappa_n$ is zero also, this implies that $h(\con,\con) = 0$, so both principal curvatures must be zero on $\partial\Sigma$. 
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%% I still think this is correct, but my collaborator disagrees.  May return to it sometime in the future. %%%%%%%%%%%%%%%%%%%%%

% \textcolor{red}{Lemma~\ref{lem:bndryctrl} gives conditions that are sufficient to severely restrict a functional $\mathcal{W}$ which is known to be nowhere scaling-invariant. First, there is the following elementary Lemma.
% \begin{lemma}\label{lem:formain2}
% Let $\mathcal{W}$ be a nowhere-scaling-invariant functional, and $\Sigma$ be any surface.  If the differential equation $2F - HF_H - 2KF_K = 0$ is satisfied pointwise on $\Sigma$, then $F\equiv 0$ on $\Sigma$.
% \end{lemma}
% \begin{proof}
% Choose a regular point $x_0\in\Sigma$ and let $H_{x_0},K_{x_0}$ denote respectively the values of the mean and Gauss curvatures at $x_0$. Let $F_0 = F(H_{x_0}, K_{x_0})$, and consider an $(H,K)$-neighborhood $U$ around $(H_{x_0},K_{x_0})$ and a curve $\Gamma:(-\varepsilon,\varepsilon)\to U$, such that $\Gamma(t) = \left( H_0(t), K_0(t) \right)$ and $\Gamma(0) = (H_{x_0},K_{x_0})$.  We will examine the local solutions to $2F - HF_H - 2KF_K = 0$ in $U$.  Consider the characteristic curves for this semilinear differential equation, which we may assume are transverse to $\Gamma$ and foliate $U$.  Then, for each curve $\sigma(s) \subset U$ there is precisely one intersection point $\sigma(0) = \Gamma(t_0)$.  Moreover, the following system of equations is satisfied in $U$:
% \begin{align*}
%     H_s(t,s) &= H(t,s), \\
%     K_s(t,s) &= 2K(t,s), \\
%     F_s(t,s) &= 2F(t,s).
% \end{align*}
% From this, it follows that
% \begin{align*}
%     H(t,s) &= H_0(t)e^s, \\
%     K(t,s) &= K_0(t)e^{2s}, \\
%     F(t,s) &= F_0(t)e^{2s}.
% \end{align*}
% Now, note that if both of $H$ and $K$ are 0 at some point of $U$, then $F=0$ there as well.  So, we may assume (perhaps after restriction) that at least one of $H,K$ is locally nonzero on $U$, say $H$.  In this case, the transversality of $\Gamma$ implies that the columns of the Jacobian $\partial(H,K)/\partial(s,t)$ are linearly independent, so the expressions for $H,K$ above may be locally inverted to yield functions $t(H,K),s(H,K)$ on $U$.  This in turn provides the local representation of $F$, \[F(H,K) = G_0\left(\frac{K}{H^2}\right) H^2,\] where $G_0 = \left(1/H_0^2\right)\left( F_0 \circ (K_0/H_0^2)^{-1}\right)$.
% On the other hand, consider a neighborhood $V \subset \Sigma$ which contains $x_0$ and whose image under $H$ and $K$ lies in $U$, which can always be found since $H$ and $K$ vary smoothly on $\Sigma$.  Since $\mathcal{W}$ is nowhere scaling-invariant, the above expression for $F$ cannot possibly hold on $U$, hence it also cannot hold on $V$.  Therefore, the only alternative is that $F\equiv 0$ on $V$.  Since the point $x_0\in\Sigma$ was arbitrary, it follows by continuity that $F\equiv 0$ on $\Sigma$.
% \end{proof}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

It is now appropriate to give the proof of Theorem~\ref{thm:main2}, which details a situation where conditions on the boundary of a $\mathcal{W}$-critical surface can exert control over the interior.

% behavior on the interior of a $\mathcal{W}$-critical surface.

% details one example of how the boundary behavior of a $\mathcal{W}$-critical surface can exert significant control over what happens in the interior.  Indeed, without dilation invariance to absorb the integration over the interior, the boundary conditions above are sufficient to impose great restrictions on the functional.

% \begin{proposition}\label{prop:formain2}
% Suppose $\mathcal{W}$ is a functional which is not scaling-invariant, and let $\*r$ be a $\mathcal{W}$-critical immersion of the surface $\Sigma$ such that:
% \begin{enumerate}
%     \item The conditions (\ref{eq:bcond1}), (\ref{eq:bcond2}), and (\ref{eq:bcond3}) are satisfied on $\partial\Sigma$,
%     \item The quantity $2F - H F_H - 2K F_K$ does not change sign on $\Sigma$.
% \end{enumerate}
% Then, $F\equiv 0$ on $\Sigma$.
% \end{proposition}

\begin{proof}[Proof of Theorem~\ref{thm:main2}]
It follows from the hypotheses and Lemma~\ref{lem:bndryctrl} that any critical surface $\Sigma$ must satisfy the integral equality \[\int_\Sigma \left(2F - HF_H - 2KF_K\right) d\mu = 0.\]  However, $\mathcal{W}$ is assumed to be shrinking or expanding, so the integrand is vanishing. 
\end{proof}

% Since the functional is either expanding or shrinking, this integrand does not change sign, so it follows that $2F - H F_H - 2K F_K = 0$ pointwise on $\Sigma$.  Since $\mathcal{W}$ is nowhere scaling-invariant, it follows \textcolor{red}{from Lemma~\ref{lem:formain2} that $F$ must be identically $0$ on $\Sigma$.} 


\subsection{Corollaries}
With Theorem~\ref{thm:main2} now established, some interesting corollaries can be extracted.  First, consider the case where $\Sigma$ has an axis of rotational symmetry.
\begin{corollary}\label{cor:main2}
Let $\mathcal{W}$ be either shrinking or expanding, and let $\Sigma$ be a rotationally-symmetric $\mathcal{W}$-surface with boundary. Suppose additionally that the following hold:
\begin{enumerate}[noitemsep]
\item $F-h(\con, \con)F_H-KF_K=0$ on $\partial\Sigma$,
\item $\nabla_\eta F_H + \kappa_n \nabla_\eta F_K = 0$ on $\partial\Sigma$.
\end{enumerate}
Then, either $\Sigma$ is spherical or there is a constant $c$ such that $F_H\equiv 0$, $F_K\equiv c$, and $F\equiv cK$ on $\Sigma$.

% Then, either $\mathcal{W}$ is scaling-invariant, or $F_H=F_K=F\equiv 0$ on $\Sigma$.
\end{corollary}

\begin{proof}
Since $\Sigma$ is rotationally-symmetric by assumption, its boundaries are lines of curvature.  As such, $\tau_g \equiv 0$ on $\partial\Sigma$, hence (\ref{eq:bcond1}) is satisfied. The result then follows from Theorem \ref{thm:main2} and Lemma \ref{lem:Vis0}. 
\end{proof}
\begin{remark}\label{rem:counterex}
	For example, the first case occurs when $F=(H^2-4K)^2$, while the second case happens if $F=H^4+K$ and $\Sigma$ is minimal.  
\end{remark}

Moreover, it is worthwhile to consider functionals which are independent of the Gauss curvature $K$, as many of these objects appear quite naturally in practice, e.g. the surface area, total mean curvature, and (non-conformal) Willmore functionals.  To that end, there is the following Corollary which details the case where $F = F(H)$ is a real analytic function of $H$ alone. 
\begin{corollary}\label{cor:minimal}
Let $\mathcal{W}$ be expanding or shrinking, $\Sigma$ be a $\mathcal{W}$-critical surface, and $F = F(H)$ be a real analytic function of $H$ alone.  Suppose $F = F_H = \nabla_\con F_H = 0$ on $\partial\Sigma$.  Then, one of the following holds:
\begin{enumerate}
    \item $F \equiv 0$ everywhere,
    \item $F \equiv cH^2$ for some $c\in\mathbb{R}$ and $\mathcal{W}$ is scaling-invariant,
    \item $\Sigma$ has constant mean curvature and $F = 0$ on $\Sigma$.
\end{enumerate}
\end{corollary}

\begin{proof}
    Notice that the system in Lemma~\ref{lem:bndryctrl} is satisfied under these assumptions.  Hence, it must follow that 
    \[\int_\Sigma \left(2F-HF_H\right)d\mu = 0.\]
    Since $\mathcal{W}$ is either shrinking or expanding, this implies that $2F-HF_H = 0$ pointwise on $\Sigma$.  If $H$ is not constant on $\Sigma$, then this equation is satisfied on a dense set of $H$-values, so either $F \equiv cH^2$ for some $c$ or $F \equiv 0$ by analyticity.  Otherwise, $\Sigma$ has constant mean curvature, and $F = 0$ on $\partial\Sigma$ implies that $F \equiv 0$ on $\Sigma$.
\end{proof}

\begin{remark}
If $F$ is assumed to be smooth instead of analytic, the conclusions of Corollary~\ref{cor:minimal} remain true only in a local sense.  That is, either $F = cH^2$ or $F = 0$ pointwise on $\Sigma$, but this need not extend to the whole domain of $\mathcal{W}$.  To see this, take for example $F(H) = \varphi(H)\, H^2$, where $\varphi(H)$ is a smooth bump function which is identically 1 on $[-1,1]$ and supported on $[-\sqrt{2}, \sqrt{2}]$ (see \cite[Chapter 13]{tu2010} for a construction).  In this case, one can verify that $2F - HF_H \geq 0$ everywhere, so $\mathcal{W}$ is expanding, and also that all derivatives of $\varphi$ vanish on $[-1,1]$.  This means that the Clifford torus $\Sigma \subset \mathbb{R}^3$ which has been rescaled so that its mean curvature lies in $[-1,1]$ is critical for $\mathcal{W}$, and (vacuously) satisfies the boundary conditions in Corollary~\ref{cor:minimal}.  However, $\mathcal{W}$ is certainly not scaling-invariant nor identically zero on its domain.  
\end{remark}
% \begin{remark}
% Other results of this form can be deduced by considering different boundary conditions.
% \end{remark}

This particular Corollary can be used to show that, in some cases, minimizers of a $\mathcal{W}$-functional can only be minimal surfaces.  In particular, for a surface with boundary $\Sigma \subset \mathbb{R}^3$ there is the 
notion of p-Willmore energy mentioned in the Introduction,
\begin{equation*}
    \mathcal{W}^p(\*r) = \int_{\*r(\Sigma)} |H|^p\, d \mu \qquad p\in\mathbb{R}.
\end{equation*}
Clearly, this coincides up to a constant factor with the usual, scaling-invariant, definition of the (non-conformal) Willmore energy when $p=2$.  On the other hand, this functional is not scaling-invariant for $p\neq 2$, since
\begin{equation*}
    2F - HF_H - 2KF_K = 2|H|^p - H\, \partial_H\left((H^2)^{p/2}\right) = (2-p)|H|^p \neq 0.
\end{equation*}
As seen before, this lack of scaling invariance has significant consequences on the critical surfaces of $\mathcal{W}^p$.  In particular, we observe that conditions on the boundary of a p-Willmore surface when $p>2$ exert much more control over what happens in the interior when compared to the case $p=2$.  To illustrate this, first note that the flux formula (\ref{eq:scaleflux}) reduces immediately to
\begin{equation}\label{eq:pwillflux}
\begin{split}
    &(2-p)\int_\Sigma |H|^p\, d\mu \\
    &= \int_{\partial\Sigma} \Big(|H|^p\langle \*r,\con\rangle + p|H|^{p-2}\left(H\nabla_\con\langle \*r,\*n\rangle - (p-1)\langle \*r,\*n\rangle \nabla_\con H \right)\Big)\, ds.
\end{split}
\end{equation}
% \begin{equation}\label{eq:pwillflux}
% \resizebox{0.99\hsize}{!}{%
%     $(2-p)\int_\Sigma |H|^p\, d\mu = \int_{\partial\Sigma} \Big(|H|^p\langle \*r,\con\rangle + p|H|^{p-2}\left(H\nabla_\con\langle \*r,\*n\rangle - (p-1)\langle \*r,\*n\rangle \nabla_\con H \right)\Big)\, ds.$%
%     }
% \end{equation}
Corollary~\ref{cor:minimal} can now be applied to establish the statement of Theorem~\ref{thm:pWillmore}.


% consequence of Corollary~\ref{fluxformula}.
% \begin{proposition}\label{pwillflux}
% The following flux formula holds.
%     \begin{equation*}
%     (2-p)\int_\Sigma |H|^p\, d\mu = \int_{\partial\Sigma} \Big(|H|^p\langle \*r,\con\rangle + p|H|^{p-2}\left(H\nabla_\con\langle \*r,\*n\rangle - (p-1)\langle \*r,\*n\rangle \nabla_\con H \right)\Big)\, ds.
% \end{equation*}
% \end{proposition}
% \begin{proof}
% Let $p = 2q$, then we have $F= |H|^p = (H^2)^{p/2} = H^{2q}$ and
% \begin{equation*}
% \begin{split}
%     &\int_{\partial\Sigma} \Big((F_H+HF_K)\nabla_\con \left\langle{\*r, \*n}\right\rangle -F_K h(\nabla \left\langle{\*r, \*n}\right\rangle, \con)\Big)\, ds\\
%     &+\int_{\partial \Sigma} \left\langle{\*r, \*n}\right\rangle\Big(h(\nabla F_K, \con)-\nabla_\con F_H-H\nabla_\con F_K\Big)\, ds+\int_{\partial \Sigma} F\left\langle{\*r, \con}\right\rangle\, ds \\
%     &= \int_{\partial\Sigma} 2q\left(H^{2q-1}\nabla_\con \langle \*r,\*n\rangle -\langle \*r,\*n\rangle \nabla_\con(H^{2q-1})\right)ds + \int_{\partial\Sigma} H^{2q}\langle \*r,\con\rangle\,ds.
% \end{split}
% \end{equation*}
% Moreover, it was computed above that
% \begin{equation*}
%     \int_\Sigma (2F - HF_H - 2KF_K) \, d\mu = (2-p)\int_\Sigma |H|^p\, d\mu.
% \end{equation*}
% Combining these two expressions in view of the middle equation in Corollary~\ref{fluxformula} then yields the conclusion.
% \end{proof}

% As mentioned before, boundary data has a strong effect on p-Willmore surfaces due to their lack of scaling invariance in general.  Impressively, it is observed in some cases that what happens on the boundary completely controls what happens inside, as seen in the following Theorem.  

% \begin{proposition}
% When $p>2$, any p-Willmore surface $\Sigma$ with boundary which satisfies $H=0$ on $\partial\Sigma$ must be a minimal surface.
% \end{proposition}
\begin{proof}[Proof of Theorem~\ref{thm:pWillmore}]
By Corollary~\ref{cor:minimal}, it is sufficient to consider 
\[|H|^p = p|H|^{p-2}H = p(p-1)H^{p-2}\nabla_\con H = 0 \quad\text{on}\,\,\partial\Sigma,\]
which is clearly satisfied under the hypothesis that $p>2$ and $H = 0$ on the boundary.  Since $|H|^p$ is not scaling-invariant for $p\neq 2$, it follows that $|H|^p \equiv 0$ on $\Sigma$.  Hence, $H\equiv 0$ and $\Sigma$ must be minimal.
\end{proof}

\begin{remark}
This result can also be deduced directly from (\ref{eq:pwillflux}) without appealing to Corollary~\ref{cor:minimal}, as the flux formula (\ref{eq:pwillflux}) reduces to
    \begin{equation*}
        \int_\Sigma |H|^p = 0,
    \end{equation*}
implying that $|H|\equiv 0$ on $\Sigma$ by continuity.
\end{remark}

\begin{remark}
Note that it is possible to show in a completely analogous fashion that there are no closed p-Willmore surfaces $\Sigma$ immersed in $\mathbb{R}^3$ when $p>2$.  Indeed, equation (\ref{eq:pwillflux}) asserts that any such surface must be minimal, but there are no closed minimal surfaces immersed in $\mathbb{R}^3$, a contradiction.
\end{remark}

Clearly this is quite different from the Willmore case of $p=2$, where there are many known and non-minimal solutions to the same boundary-value problem (e.g. \cite{deckelnick2009}).  It is likely true that other $\mathcal{W}$-functionals which lack scale-invariance are similarly influenced by their boundary data, but this is a study for future work.  It is hoped that the results and Corollaries developed here will be of use in answering such questions.

